A Theory of Ex Post Rationalization

People rationalize their past choices, even those that were mistakes in hindsight. We propose a formal theory of this behavior. The theory predicts that sunk costs affect later choices. Its model primitives are identified by choice behavior and it yields tractable comparative statics.

==> Subfiles/3_evidence_backup.tex <==
\section{Evidence on \textit{ex post} rationalization}\label{sec:evidence}

\subsection{Evidence from psychology}\label{sec:psych_evidence}

We review psychological research pertinent to the present theory. We cover only a fraction of the vast literature on rationalization; as \cite{cushman2020rationalization} writes, ``Among psychologists, [rationalization] is one of the most exhaustively documented and relentlessly maligned acts in the human repertoire." 

The present theory posits that the agent evaluates the past from the \textit{ex post} perspective, as is consistent with the literature on hindsight bias. This literature finds that after an event has occurred, people are overconfident that they could have predicted it in advance \citep{fischhoff1975hindsight,blank2007hindsight}, and even misremember their own \textit{ex ante} predictions, falsely believing that they predicted what came to pass \citep{fischhoff1975knew, fischhoff1977perceived}. Hence, it is plausible that people adopt the \textit{ex post} rather than the \textit{ex ante} perspective when evaluating their past choices.

In the present theory, rather than sticking to her original motives, the agent adopts \textit{post hoc} rationales that justify her actions. The psychology literature on confabulation finds that people generate \textit{post hoc} rationales and sincerely believe them. Confabulation has been documented in split-brain patients \citep{gazzaniga1967split, gazzaniga2005forty} and in ordinary people manipulated to misremember what they chose \citep{johansson2005failure, johansson2006something}. \cite{nisbett1977telling} find that subjects are often unaware of the effects of experimental stimuli on their behavior, and offer spurious explanations when queried by experimenters.

Cognitive dissonance theory posits that people adapt their cognitions so as to achieve internal consistency \citep{festinger1957theory}.  In particular, they adapt their attitudes and beliefs to justify their past choices.  A variety of experiments find evidence for this hypothesis.  When a reading group conducts an unexpectedly humiliating initiation ritual, this causes new members to evaluate the group more positively, a result due to \cite{aronson1959effect} and replicated by \cite{gerard1966effects}.  The mere fact that an alternative was chosen in the past causes lab subjects to evaluate it more positively and causes them to be more likely to choose it in future \citep{arad2013past}.\footnote{This result originates from the experiment of \cite{brehm1956postdecision}, which is confounded by self-selection bias \citep{chen2010choice,risen2010study}. \cite{arad2013past} modified the paradigm to remove the confound.} \cite{harmon2007cognitive} review the substantial experimental evidence on cognitive dissonance.

In summary, the mental mechanisms behind \textit{ex post} rationalization have been studied by psychologists for decades. Our contribution is to formalize these in a tractable economic model.

\subsection{Sunk costs and foregone benefits}\label{sec:sunk_costs}

Sunk-cost effects have been documented in many settings, including  business decisions \citep{staw1976knee, mccarthy1993reinvestment,schoorman1988escalation,staw1997escalation}, usage of durable goods \citep{ho2018sunk}, professional sports \citep{staw1995sunk,camerer1999econometrics,keefer2017sunk}, and auctions \citep{herrmann2015beating,augenblick2016sunk}.  Some studies find no evidence of sunk-cost effects \citep{ashraf2010can,friedman2007searching,ketel2016tuition,negrini2020still}.\footnote{For a meta-analysis, see \cite{roth2015sunk}}

Despite the intuitive pull of sunk-cost effects and their clear relevance to economic decisions, there is no workhorse theory of sunk-cost effects with broad scope. Most empirical analyses of sunk costs either do not test a formal theory of sunk-cost effects or use bespoke theories designed for particular contexts.\footnote{Of the studies cited above, \cite{staw1976knee}, \cite{mccarthy1993reinvestment}, \cite{schoorman1988escalation}, \cite{staw1997escalation}, \cite{staw1995sunk}, \cite{camerer1999econometrics}, \cite{keefer2017sunk}, \cite{herrmann2015beating}, \cite{friedman2007searching}, and \cite{ketel2016tuition} do not test a formal theory of sunk costs. \cite{ho2018sunk} and \cite{augenblick2016sunk} test theories specialized to durable goods and dynamic auctions respectively. \cite{negrini2020still} test the predictions of cumulative prospect theory \citep{tversky1992advances}, and do not find evidence that it drives sunk-cost effects. \cite{ashraf2010can} test the taste-for-consistency theory of \cite{eyster2002rationalizing}.}

\textit{Ex post} rationalization is a candidate for a workhorse theory.  It predicts that sunk-cost effects will occur when the agent has made an \textit{ex post} mistake that can be rationalized by doubling down on the original course of action.

Sunk-cost effects do not rely on the functional form we chose for \Cref{ex:baseline}. Instead, consider an agent making a risky investment decision to invent a new product.  He chooses investment levels $a_1,a_2 \in [0,1]$.  The project succeeds with probability $\phi(a_1,a_2)$, where $\phi$ is increasing in both arguments, differentiable, and has a positive cross-partial derivative. The agent's rationales involve adapting his belief about the expected profits conditional on success; this is captured by $\theta \in \mathbb{R}$.  His payoff under rationale $v_\theta$ is
\begin{equation}
    \theta \phi(a_1,a_2) - s a_1 - a_2.
\end{equation}
$s$ is a non-negative shock to time-$1$ investment costs. These costs are sunk at time $2$, so a classical agent's time-$2$ choice does not depend on $s$. By contrast, for an \textit{ex post} rationalizer, high time-$1$ cost shocks lead to higher time-$2$ investments.

More broadly, suppose that the agent's rationales involve adapting his value $\theta$ for consuming some good or achieving some goal. In \Cref{sec:comp_stat}, we find that sunk-cost effects are implied by a general comparative statics result, that applies whenever the agent's payoffs are supermodular in $a_1$, $a_2$, and $\theta$.  Supermodularity is a standard condition that captures complementarity between choice variables.

In models with limited memory, self-signaling can induce sunk-cost effects, because the agent's time-$1$ action signals her time-$1$ information to her time-$2$ self \citep{baliga2011mnemonomics, hong2019sunk}. \cite{baliga2011mnemonomics} find in a lab experiment that sunk-cost effects arise even without memory limitations, and argue that in these situations sunk-cost effects are a well-adapted default heuristic. In light of this, we suggest it is useful to have a simple model of the resulting behavior that abstracts from the intricacies of self-signaling equilibria.

Reputation concerns can give rise to sunk-cost effects. For instance, a project manager might respond to sunk costs so as to convince the market that he is competent \citep{prendergast1996impetuous}, and agents in bilateral relationships might respond to sunk costs so as to improve their reputation for future partners \citep{mcafee2010sunk}. The present model can be seen as a tractable reduced form for reputation concerns, as in \Cref{sec:justif_to_others}.  Its simple linear form abstracts from the details of signaling equilibria, and in return allows the theory to apply to a wider class of decision problems. However, the evidence of \Cref{sec:psych_evidence} suggests that rationalization is a basic psychological process, operating even in situations without reputation concerns or memory limitations.

Reference-dependent preferences are an alternative explanation for sunk-cost effects \citep{thaler1980toward, arkes1985psychology}. Returning to \Cref{ex:baseline}, if Bob buys the ticket and stays home in the snowstorm, then this results in a sure loss relative to his reference point. On the other hand, attending the game in a snowstorm is a gain in some dimensions and a loss in others.  The standard prospect theory value function is convex over losses \citep{kahneman1979prospect}, which can lead Bob to attend the game after buying the ticket, but to stay home if the ticket was free.

\textit{Ex post} rationalization and reference-dependence make different predictions about \Cref{ex:nochoice}, in which Bob receives a ticket and loses \$100 through no choice of his own.  The usual way to close the reference-dependent model is to use the agent's expectations to set the reference point, as in \cite{kHoszegi2006model}.  For any personal equilibrium in which Bob buys the ticket for \$100 in \Cref{ex:baseline}, his reference point is the same as in \Cref{ex:nochoice}. Thus, expectations-based reference dependence (EBRD) is constrained to predict the same time-$2$ behavior regardless of whether Bob made a choice to buy the ticket. By contrast, \textit{ex post} rationalization predicts that Bob's time-$2$ decision depends on whether he could have chosen otherwise at time $1$.

Recent work finds that sunk-cost effects depend on whether the decision-maker was responsible for incurring those costs, as predicted by \textit{ex post} rationalization. \cite{martens2021escalating} study the effect of sunk costs on follow-up investment decisions, in a laboratory experiment. They find that sunk-cost effects increase substantially when subjects are responsible for the initial investment decision. Similarly, \cite{guenzel2021too} studies high-stakes corporate acquisitions and finds that exogenous cost shocks (occurring \textit{after} the acquisition decision) decrease the acquiring company's willingness to divest, but this effect is much reduced if the CEO who led the acquisition steps down.

One novel prediction of \textit{ex post} rationalization is that it generates `foregone-benefit' effects, as in the following example:
\begin{example}\label{ex:foregone_benefit}
Bob must choose between a free ticket to the game and a bet that pays \$100 if Seabiscuit wins the horse race (and \$0 otherwise). Bob chooses the free ticket and hence foregoes the bet.  Seabiscuit wins the race. On the day of the game there is a snowstorm. Bob attends the game, but if instead Seabiscuit had lost, Bob would have stayed home.
\end{example}
After choosing the ticket, a rational agent can ignore whether Seabiscuit won the race. Foregone benefits cannot be acquired, just as sunk costs cannot be recouped, so they have no effect on time-$2$ incentives.  By contrast, an \textit{ex post} rationalizer with the same parameters posited in \Cref{sec:intro} also exhibits the behavior in \Cref{ex:foregone_benefit}.

More generally, when a rationalizer foregoes some uncertain benefit in order to pursue a course of action, higher realizations of the benefit cause him to double down on that course of action.\footnote{The sunk-cost and foregone-benefit effects are both implied by the conclusion of \Cref{thm:comp_stat}.}

The behavior in \Cref{ex:foregone_benefit} is not consistent with reference dependence, for any standard method to set reference points. Bob chose the ticket, so his expectations about time-$2$ consumption depend not at all on the race. \cite{kahneman1979prospect} propose setting the reference point at the status quo or at `current assets'. Bob's pre-decision status quo (holding neither ticket nor the bet) does not depend on the race.  After choosing the ticket, Bob's current assets do not depend on whether Seabiscuit wins. In this way, decision problems with foregone benefits cleanly distinguish between reference dependence and \textit{ex post} rationalization.

==> tikzlibrarytikzmark.code.tex <==
%%
%% This is file `tikzlibrarytikzmark.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tikzmark.dtx  (with options: `tikzlibrary')
%% ----------------------------------------------------------------
%% tikzmark --- remembering absolute positioning with TikZ.
%% E-mail: loopspace@mathforge.org
%% Released under the LaTeX Project Public License v1.3c or later
%% See http://www.latex-project.org/lppl.txt
%% ----------------------------------------------------------------
%% 
\ProvidesFile{tikzlibrarytikzmark.code.tex}[%
  2021/02/16
  v1.10
  TikZ library for marking positions in a document]
\RequirePackage{expl3, l3keys2e, xparse}
\tikzset{%
  remember picture with id/.style={%
    remember picture,
    overlay,
    save picture id=#1,
  },
  every picture/.append style={%
    execute at end picture={%
      \ifpgfrememberpicturepositiononpage%
      \edef\pgf@temp{%
        \noexpand\write\noexpand\pgfutil@auxout{%
          \string\savepicturepage%
          {\pgfpictureid}{\noexpand\arabic{page}}%
        }%
      }%
      \pgf@temp
      \fi%
    },
  },
  check picture id/.code={
    \ifpgfrememberpicturepositiononpage
    \@ifundefined{pgf@sys@pdf@mark@pos@\pgfpictureid}{%
      \tikzset{%
        name prefix/.get=\tzmk@name@prefix,
        name prefix/.prefix=discard-,
        execute at end picture={%
          \tikzset{name prefix/.expand once=\tzmk@name@prefix}%
        },
      }%
    }{}%
    \fi
  },
  maybe define node/.style={%
    execute at end picture={%
      \ifpgfrememberpicturepositiononpage
      \@ifundefined{pgf@sh@pi@\tikz@pp@name{#1}}{%
        \pgfnodealias{\tikz@pp@name{#1}}{discard-\tikz@pp@name{#1}}%
      }{}%
      \fi
    }%
  },
  save picture id/.code={%
      \protected@write\pgfutil@auxout{}{%
      \string\savepointas%
      {\tikzmark@pp@name{#1}}{\pgfpictureid}{0pt}{0pt}}%
  },
  if picture id/.code args={#1#2#3}{%
    \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
      \pgfkeysalso{#3}%
    }{
      \pgfkeysalso{#2}%
    }
  },
  next page/.is choice,
  next page vector/.initial={\pgfqpoint{0pt}{0pt}},
  next page/below/.style={%
    next page vector={\pgfqpoint{0pt}{-\the\paperheight}}%
  },
  next page/above/.style={%
    next page vector={\pgfqpoint{0pt}{\the\paperheight}}%
  },
  next page/left/.style={%
    next page vector={\pgfqpoint{-\the\paperwidth}{0pt}}%
  },
  next page/right/.style={%
    next page vector={\pgfqpoint{\the\paperwidth}{0pt}}%
  },
  next page/ignore/.style={%
    next page vector={\pgfqpoint{0pt}{0pt}}%
  },
  if tikzmark on current page/.code n args={3}{%
    \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
      \pgfkeysalso{#3}%
    }{%
      \@ifundefined{%
        save@pg@\csname save@pt@\tikzmark@pp@name{#1}\endcsname
      }{%
        \pgfkeysalso{#3}%
      }{%
        \ifnum\csname save@pg@%
        \csname save@pt@\tikzmark@pp@name{#1}\endcsname%
        \endcsname=\the\value{page}\relax%
        \pgfkeysalso{#2}%
        \else
        \pgfkeysalso{#3}%
        \fi
      }%
    }%
  },
  if tikzmark on page/.code n args={4}{%
    \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
      \pgfkeysalso{#4}%
    }{%
      \@ifundefined{%
        save@pg@\csname save@pt@\tikzmark@pp@name{#1}@label\endcsname%
      }{%
        \pgfkeysalso{#4}%
      }{%
        \ifnum\csname save@pg@%
        \csname save@pt@\tikzmark@pp@name{#1}\endcsname%
        \endcsname=#2\relax%
        \pgfkeysalso{#3}%
        \else
        \pgfkeysalso{#4}%
        \fi
      }%
    }%
  },
  tikzmark prefix/.initial=,%
  tikzmark suffix/.initial=,%
}
\def\tikzmark@pp@name#1{%
  \csname pgfk@/tikz/tikzmark prefix\endcsname%
  #1%
  \csname pgfk@/tikz/tikzmark suffix\endcsname%
}%
\def\savepointas#1#2#3#4{%
  \expandafter\gdef\csname save@pt@#1\endcsname{#2}%
  \expandafter\gdef\csname save@pt@#1@offset\endcsname%
  {\pgfqpoint{#3}{#4}}%
}
\def\savepicturepage#1#2{%
  \expandafter\gdef\csname save@pg@#1\endcsname{#2}%
}
\def\tikzmarkalias#1#2{%
  \pgf@node@gnamelet{save@pt@#1}{save@pt@#2}%
  \pgf@node@gnamelet{save@pt@#1@offset}{save@pt@#2@offset}%
}
\def\tmk@labeldef#1,#2\@nil{%
  \edef\tmk@label{\tikzmark@pp@name{#1}}%
  \def\tmk@def{#2}%
}
\tikzdeclarecoordinatesystem{pic}{%
  \pgfutil@in@,{#1}%
  \ifpgfutil@in@%
    \tmk@labeldef#1\@nil
  \else
    \tmk@labeldef#1,(0pt,0pt)\@nil
  \fi
  \@ifundefined{save@pt@\tmk@label}{%
    \tikz@scan@one@point\pgfutil@firstofone\tmk@def
  }{%
    \pgfsys@getposition{\csname save@pt@\tmk@label\endcsname}%
    \save@orig@pic%
    \pgfsys@getposition{\pgfpictureid}\save@this@pic%
    \pgf@process{\pgfpointorigin\save@this@pic}%
    \pgf@xa=\pgf@x
    \pgf@ya=\pgf@y
    \pgf@process{\pgfpointorigin\save@orig@pic}%
    \advance\pgf@x by -\pgf@xa
    \advance\pgf@y by -\pgf@ya
    \pgf@xa=\pgf@x
    \pgf@ya=\pgf@y
    \pgf@process%
    {\pgfpointorigin\csname save@pt@\tmk@label @offset\endcsname}%
    \advance\pgf@xa by \pgf@x
    \advance\pgf@ya by \pgf@y
      \@ifundefined{save@pg@\csname save@pt@\tmk@label\endcsname}{}{%
        \@ifundefined{save@pg@\pgfpictureid}{}{%
          \pgfkeysvalueof{/tikz/next page vector}%
        \edef\tmk@pg{%
          \the\numexpr \csname save@pg@%
          \csname save@pt@\tmk@label\endcsname\endcsname%
          -
          \csname save@pg@\pgfpictureid\endcsname\relax%
        }%
        \ifnum \tmk@pg > 0 \relax
        \advance \pgf@xa by \pgf@x\relax
        \advance \pgf@ya by \pgf@y\relax
        \fi
        \ifnum \tmk@pg < 0 \relax
        \advance \pgf@xa by -\pgf@x\relax
        \advance \pgf@ya by -\pgf@y\relax
        \fi
        }%
      }%
      \pgf@x=\pgf@xa
      \pgf@y=\pgf@ya
    \pgftransforminvert
    \pgf@pos@transform{\pgf@x}{\pgf@y}%
  }%
}
\newcommand\tikzmark@outside[2][]{%
\tikzset{external/export next/.try=false}%
\tikz[remember picture with id=#2]{#1}%
}
\def\tikzmark@inside#1#2{%
  \tikzset{remember picture}%
  \tikz@scan@one@point\pgfutil@firstofone#2\relax
  \protected@write\pgfutil@auxout{}{%
    \string\savepointas%
    {\tikzmark@pp@name{#1}}{\pgfpictureid}{\the\pgf@x}{\the\pgf@y}}%
}
\def\tikzmark{%
  \ifx\pgfpictureid\@undefined
  \let\tikzmark@next=\tikzmark@outside
  \else
  \relax
  \ifx\scope\tikz@origscope\relax
  \let\tikzmark@next=\tikzmark@outside
  \else
  \let\tikzmark@next=\tikzmark@inside
  \fi
  \fi
  \tikzmark@next%
}
\newcommand\pgfmark[1]{%
    \bgroup
    \global\advance\pgf@picture@serial@count by1\relax%
    \edef\pgfpictureid{pgfid\the\pgf@picture@serial@count}%
      \pgfsys@markposition{\pgfpictureid}%
    \edef\pgf@temp{%
      \noexpand\write\noexpand\pgfutil@auxout{%
        \string\savepicturepage{\pgfpictureid}{\noexpand\arabic{page}}}}%
    \pgf@temp
    \protected@write\pgfutil@auxout{}{%
      \string\savepointas{\tikzmark@pp@name{#1}}{\pgfpictureid}{0pt}{0pt}}%
    \egroup
  }
\@ifclassloaded{beamer}{
  \renewcommand<>{\tikzmark@outside}[2][]{%
    \only#3{\beameroriginal{\tikzmark@outside}[{#1}]{#2}}%
  }
  \renewcommand<>{\tikzmark@inside}[2]{%
    \only#3{\beameroriginal{\tikzmark@inside}{#1}{#2}}%
  }
}{}
\@ifclassloaded{beamer}{
  \renewcommand<>{\pgfmark}[1]{\only#2{\beameroriginal{\pgfmark}{#1}}}
}{}
\@ifclassloaded{beamer}{
  \tikzset{
    tikzmark suffix=-\the\beamer@slideinframe
  }
}{}
\newif\iftikzmark@
\newcommand\iftikzmark[3]{%
    \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
      #3%
    }{%
      #2%
    }%
}%
\newcommand\iftikzmarkexists[1]{%
  \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
    \tikzmark@false%
  }{%
    \tikzmark@true%
  }%
  \iftikzmark@
}%
\newcommand\iftikzmarkonpage[2]{%
  \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
    \tikzmark@false
  }{%
    \@ifundefined{save@pg@\csname save@pt@\tikzmark@pp@name{#1}\endcsname}{%
      \tikzmark@false
    }{%
      \ifnum\csname save@pg@%
      \csname save@pt@\tikzmark@pp@name{#1}\endcsname%
      \endcsname=#2\relax%
      \tikzmark@true
      \else
      \tikzmark@false
      \fi
    }%
  }%
  \iftikzmark@
}
\newcommand\iftikzmarkoncurrentpage[1]{%
  \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
    \tikzmark@false
  }{%
    \@ifundefined{save@pg@\csname save@pt@\tikzmark@pp@name{#1}\endcsname}{%
      \tikzmark@false
    }{%
      \ifnum\csname save@pg@%
      \csname save@pt@\tikzmark@pp@name{#1}\endcsname%
      \endcsname=\the\value{page}\relax%
      \tikzmark@true
      \else
      \tikzmark@false
      \fi
    }%
  }%
  \iftikzmark@
}
\def\subnode@#1#2#3{%
  \begingroup
  \pgfmark{#2}%
  \setbox\pgfnodeparttextbox=\hbox\bgroup #3\egroup
  \def\tikz@fig@name{#2}%
  \tikzset{every subnode/.try,#1}%
  \pgfpointorigin
  \tikz@scan@one@point\pgfutil@firstofone(pic cs:#2)\relax
  \advance\pgf@x by .5\wd\pgfnodeparttextbox
  \advance\pgf@y by .5\ht\pgfnodeparttextbox
  \advance\pgf@y by -.5\dp\pgfnodeparttextbox
  \pgftransformshift{}%
  \setbox\@tempboxa=\hbox\bgroup
  {%
    \let\pgf@sh@savedmacros=\pgfutil@empty% MW
    \let\pgf@sh@savedpoints=\pgfutil@empty%
    \def\pgf@sm@shape@name{rectangle}% CJ % TT added prefix!
    \pgf@sh@s@rectangle%
    \pgf@sh@savedpoints%
    \pgf@sh@savedmacros% MW
    \pgftransformshift{%
      \pgf@sh@reanchor{rectangle}{center}%
      \pgf@x=-\pgf@x%
      \pgf@y=-\pgf@y%
    }%
    \expandafter\pgfsavepgf@process\csname pgf@sh@sa@\tikz@fig@name\endcsname{%
      \pgf@sh@reanchor{rectangle}{center}% FIXME : this is double work!
    }%
    % Save the saved points and the transformation matrix
    \edef\pgf@node@name{\tikz@fig@name}%
    \ifx\pgf@node@name\pgfutil@empty%
    \else%
    \expandafter\xdef\csname pgf@sh@ns@\pgf@node@name\endcsname{rectangle}%
    \edef\pgf@sh@@temp{%
      \noexpand\gdef\expandafter\noexpand\csname pgf@sh@np@\pgf@node@name\endcsname}%
    \expandafter\pgf@sh@@temp\expandafter{%
      \pgf@sh@savedpoints}%
    \edef\pgf@sh@@temp{%
      \noexpand\gdef\expandafter\noexpand\csname pgf@sh@ma@\pgf@node@name\endcsname}% MW
    \expandafter\pgf@sh@@temp\expandafter{\pgf@sh@savedmacros}% MW
    \pgfgettransform\pgf@temp
    \expandafter\xdef\csname pgf@sh@nt@\pgf@node@name\endcsname{\pgf@temp}%
    \expandafter\xdef\csname pgf@sh@pi@\pgf@node@name\endcsname{\pgfpictureid}%
    \fi%
  }%
  \egroup
  \box\pgfnodeparttextbox
  \endgroup
}

\newcommand\subnode[3][]{%
  \ifmmode
  \mathchoice{%
    \subnode@{#1}{#2-d}{\(\displaystyle #3\)}%
  }{%
    \subnode@{#1}{#2-t}{\(\textstyle #3\)}%
  }{%
    \subnode@{#1}{#2-s}{\(\scriptstyle #3\)}%
  }{%
    \subnode@{#1}{#2-ss}{\(\scriptscriptstyle #3\)}%
  }%
  \let\pgf@nodecallback\pgfutil@gobble
  \def\tzmk@prfx{pgf@sys@pdf@mark@pos@pgfid}%
  \edef\tzmk@pic{\tzmk@prfx\the\pgf@picture@serial@count}
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
  \edef\tzmk@pic{\tzmk@prfx\the\numexpr\the\pgf@picture@serial@count-1\relax}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
\edef\tzmk@pic{\tzmk@prfx\the\numexpr\the\pgf@picture@serial@count-2\relax}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
\edef\tzmk@pic{\tzmk@prfx\the\numexpr\the\pgf@picture@serial@count-3\relax}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
  \pgfutil@ifundefined{pgf@sh@ns@#2}{%
    \pgfnodealias{#2}{#2-t}%
    \tikzmarkalias{#2}{#2-t}%
  }{}%
  \else
    \pgfnodealias{#2}{#2-d}%
    \tikzmarkalias{#2}{#2-d}%
  \fi
  \else
    \pgfnodealias{#2}{#2-t}%
    \tikzmarkalias{#2}{#2-t}%
  \fi
  \else
    \pgfnodealias{#2}{#2-s}%
    \tikzmarkalias{#2}{#2-s}%
  \fi
  \else
    \pgfnodealias{#2}{#2-ss}%
    \tikzmarkalias{#2}{#2-ss}%
  \fi
  \else
    \subnode@{#1}{#2}{#3}%
  \fi
}

\def\tikzmarknode@#1#2#3{%
\tikzset{external/export next/.try=false}%
  \tikz[%
    remember picture,
    save picture id={#2},
    check picture id,
    maybe define node={#2},
    baseline=(#2.base),
    every tikzmarknode picture/.try
  ] {
    \node[
      anchor=base,
      inner sep=0pt,
      minimum width=0pt,
      name={#2},
      node contents={#3},
      every tikzmarknode/.try,
      #1
  ]}%
}

\newcommand\tikzmarknode[3][]{%
  \ifmmode
  \mathchoice{%
    \tikzmarknode@{#1}{#2-d}{\(\displaystyle #3\)}%
  }{%
    \tikzmarknode@{#1}{#2-t}{\(\textstyle #3\)}%
  }{%
    \tikzmarknode@{#1}{#2-s}{\(\scriptstyle #3\)}%
  }{%
    \tikzmarknode@{#1}{#2-ss}{\(\scriptscriptstyle #3\)}%
  }%
  \let\pgf@nodecallback\pgfutil@gobble
  \def\tzmk@prfx{pgf@sys@pdf@mark@pos@pgfid}%
  \edef\tzmk@pic{\tzmk@prfx\the\pgf@picture@serial@count}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
  \edef\tzmk@pic{\tzmk@prfx\the\numexpr\the\pgf@picture@serial@count-1\relax}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
\edef\tzmk@pic{\tzmk@prfx\the\numexpr\the\pgf@picture@serial@count-2\relax}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
\edef\tzmk@pic{\tzmk@prfx\the\numexpr\the\pgf@picture@serial@count-3\relax}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
  \pgfutil@ifundefined{pgf@sh@ns@\tikz@pp@name{#2}}{%
    \pgfnodealias{\tikz@pp@name{#2}}{\tikz@pp@name{#2-t}}%
    \tikzmarkalias{\tikzmark@pp@name{#2}}{\tikzmark@pp@name{#2-t}}%
  }{}%
  \else
    \pgfnodealias{\tikz@pp@name{#2}}{\tikz@pp@name{#2-d}}%
    \tikzmarkalias{\tikzmark@pp@name{#2}}{\tikzmark@pp@name{#2-d}}%
  \fi
  \else
    \pgfnodealias{\tikz@pp@name{#2}}{\tikz@pp@name{#2-t}}%
    \tikzmarkalias{\tikzmark@pp@name{#2}}{\tikzmark@pp@name{#2-t}}%
  \fi
  \else
    \pgfnodealias{\tikz@pp@name{#2}}{\tikz@pp@name{#2-s}}%
    \tikzmarkalias{\tikzmark@pp@name{#2}}{\tikzmark@pp@name{#2-s}}%
  \fi
  \else
    \pgfnodealias{\tikz@pp@name{#2}}{\tikz@pp@name{#2-ss}}%
    \tikzmarkalias{\tikzmark@pp@name{#2}}{\tikzmark@pp@name{#2-ss}}%
  \fi
  \else
    \tikzmarknode@{#1}{#2}{#3}%
  \fi
}
\def\usetikzmarklibrary{%
  \pgfutil@ifnextchar[{\use@tikzmarklibrary}{\use@@tikzmarklibrary}%
  }%}
\def\use@tikzmarklibrary[#1]{\use@@tikzmarklibrary{#1}}
\def\use@@tikzmarklibrary#1{%
  \edef\pgf@list{#1}%
  \pgfutil@for\pgf@temp:=\pgf@list\do{%
    \expandafter\pgfkeys@spdef\expandafter\pgf@temp\expandafter{\pgf@temp}%
    \ifx\pgf@temp\pgfutil@empty
    \else
      \expandafter\ifx\csname tikzmark@library@\pgf@temp @loaded\endcsname\relax%
      \expandafter\global\expandafter\let%
      \csname tikzmark@library@\pgf@temp @loaded\endcsname=\pgfutil@empty%
      \expandafter\edef\csname tikzmark@library@#1@atcode\endcsname{\the\catcode`\@}
      \expandafter\edef\csname tikzmark@library@#1@barcode\endcsname{\the\catcode`\|}
      \catcode`\@=11
      \catcode`\|=12
      \pgfutil@InputIfFileExists{tikzmarklibrary\pgf@temp.code.tex}{}{
          \PackageError{tikzmark}{I did not find the tikzmark extras library '\pgf@temp'.}{}
        }%
      \catcode`\@=\csname tikzmark@library@#1@atcode\endcsname
      \catcode`\|=\csname tikzmark@library@#1@barcode\endcsname
      \fi%
    \fi
  }%
}

\ExplSyntaxOn
\prop_new:N \g__sn_prop
\tl_new:N \l__sn_tmpa_tl
\tl_new:N \l__sn_tmpb_tl
\tl_new:N \l__open_bracket_tl
\tl_set:Nn  \l__open_bracket_tl {[} %]
\tl_new:N \l__sn_group_tl
\clist_new:N \l__sn_nodes_clist
\bool_new:N \l__sn_file_bool
\bool_new:N \g__sn_preamble_bool
\bool_set_true:N \g__sn_preamble_bool
\msg_new:nnn {tikzmark} {no file} {File~ "#1"~ doesn't~ exist.}
\msg_new:nnn {tikzmark} {loading nodes} {Loading~ nodes~ from~ "#1".}
\dim_new:N \l__sn_x_dim
\dim_new:N \l__sn_y_dim
\dim_new:N \l__sn_xa_dim
\dim_new:N \l__sn_ya_dim
\tl_new:N \l__sn_centre_tl

\tl_new:N \l__sn_transformation_tl
\tl_set:Nn \l__sn_transformation_tl {{1}{0}{0}{1}{0pt}{0pt}}
\iow_new:N \g__sn_stream
\bool_new:N \g__sn_stream_bool
\tl_new:N \g__sn_filename_tl
\tl_gset:Nx \g__sn_filename_tl {\c_sys_jobname_str}

\cs_new_nopar:Npn \sn_open_stream:
{
  \bool_if:NF \g__sn_stream_bool
  {
    \iow_open:Nn \g__sn_stream {\tl_use:N \g__sn_filename_tl .nodes}
    \bool_gset_true:N \g__sn_stream_bool
  }
}

\AtEndDocument
{
  \ExplSyntaxOn
  \bool_if:NT \g__sn_stream_bool
  {
    \iow_close:N \g__sn_stream
  }
  \ExplSyntaxOff
}
\makeatletter
\cs_set_eq:NN \tikz_set_node_name:n \tikz@pp@name
\cs_set_eq:NN \tikz_fig_must_be_named: \tikz@fig@mustbenamed

\cs_new_nopar:Npn \tikz_scan_point:n #1
{
  \tikz@scan@one@point\pgfutil@firstofone#1\relax
}

\cs_new_nopar:Npn \tikz_scan_point:NNn #1#2#3
{
  \tikz@scan@one@point\pgfutil@firstofone#3\relax
  \dim_set_eq:NN #1 \pgf@x
  \dim_set_eq:NN #2 \pgf@y
}

\makeatother
\cs_generate_variant:Nn \tikz_scan_point:n {V}
\cs_generate_variant:Nn \tikz_scan_point:NNn {NNV}
\cs_new_nopar:Npn \save_nodes:Nn #1#2
{
  \tl_clear:N \l__sn_tmpa_tl
  \tikz_scan_point:NNn \l__sn_x_dim \l__sn_y_dim {(current~ bounding~ box.center)}
  \dim_set:Nn \l__sn_x_dim {-\l__sn_x_dim}
  \dim_set:Nn \l__sn_y_dim {-\l__sn_y_dim}
  \tl_set:Nx \l__sn_centre_tl {
    {1}{0}{0}{1}{\dim_use:N \l__sn_x_dim}{\dim_use:N \l__sn_y_dim}
  }
  \clist_map_inline:nn {#2}
  {
    \tl_if_exist:cT {pgf@sh@ns@##1}
    {
      \clist_map_inline:nn {ns,np,ma,pi}
      {
        \tl_put_right:Nn \l__sn_tmpa_tl
        {
          \tl_gset:cn {pgf@sh@####1@ \tikz_set_node_name:n{##1} }
        }
        \tl_if_exist:cTF {pgf@sh@####1@##1}
        {
          \tl_put_right:Nx \l__sn_tmpa_tl {
            {\exp_not:v {pgf@sh@####1@ \tikz_set_node_name:n {##1}}}
          }
        }
        {
          \tl_put_right:Nx \l__sn_tmpa_tl {{}}
        }
      }
      \tl_put_right:Nn \l__sn_tmpa_tl
      {
        \tl_gset:cn {pgf@sh@nt@ \tikz_set_node_name:n{##1} }
      }
      \compose_transformations:NVv \l__sn_tmpb_tl \l__sn_centre_tl {pgf@sh@nt@##1}
      \tl_put_right:Nx \l__sn_tmpa_tl {{\exp_not:V \l__sn_tmpb_tl}}
      \tl_put_right:Nn \l__sn_tmpa_tl {
        \transform_node:Nn \l__sn_transformation_tl {
          \tikz_set_node_name:n{##1}
        }
      }
    }
  }
  \tl_set_eq:NN #1 \l__sn_tmpa_tl
}
\cs_new_nopar:Npn \save_nodes_to_list:nn #1#2
{
  \save_nodes:Nn \l__sn_tmpa_tl {#2}
  \prop_gput:NnV \g__sn_prop {#1} \l__sn_tmpa_tl
}
\cs_new_nopar:Npn \save_nodes_to_file:n #1
{
  \save_nodes:Nn \l__sn_tmpa_tl {#1}
  \sn_open_stream:
  \iow_now:Nx \g__sn_stream
  {
    \iow_newline:
    \exp_not:V \l__sn_tmpa_tl
    \iow_newline:
  }
}
\cs_generate_variant:Nn \save_nodes_to_list:nn {VV}
\cs_generate_variant:Nn \save_nodes_to_file:n {V}
\cs_new_nopar:Npn \restore_nodes_from_list:n #1
{
  \prop_get:NnNT \g__sn_prop {#1} \l__sn_tmpa_tl
  {
    \tl_use:N \l__sn_tmpa_tl
  }
}
\cs_new_nopar:Npn \restore_nodes_from_file:n #1
{
  \file_if_exist:nTF {#1.nodes}
  {
    \msg_log:nnn {tikzmark} {loading nodes} {#1}
    \ExplSyntaxOn
    \file_input:n {#1.nodes}
    \ExplSyntaxOff
  }
  {
    \msg_warning:nnn {tikzmark} {no file} {#1}
  }
}
\AtBeginDocument{\bool_gset_false:N \g__sn_preamble_bool}

\cs_new_nopar:Npn \compose_transformations:Nnn #1#2#3
{
  \tl_gset:Nx #1
  {
    {\fp_eval:n {
        \tl_item:nn {#2} {1}
        * \tl_item:nn {#3} {1}
        +
        \tl_item:nn {#2} {3}
        * \tl_item:nn {#3} {2}
      }
    }
    {\fp_eval:n {
        \tl_item:nn {#2} {2}
        * \tl_item:nn {#3} {1}
        +
        \tl_item:nn {#2} {4}
        * \tl_item:nn {#3} {2}
      }
    }
    {\fp_eval:n {
        \tl_item:nn {#2} {1}
        * \tl_item:nn {#3} {3}
        +
        \tl_item:nn {#2} {3}
        * \tl_item:nn {#3} {4}
      }
    }
    {\fp_eval:n {
        \tl_item:nn {#2} {2}
        * \tl_item:nn {#3} {3}
        +
        \tl_item:nn {#2} {4}
        * \tl_item:nn {#3} {4}
      }
    }
    {\fp_to_dim:n {
        \tl_item:nn {#2} {1}
        * \tl_item:nn {#3} {5}
        +
        \tl_item:nn {#2} {3}
        * \tl_item:nn {#3} {6}
        +
        \tl_item:nn {#2} {5}
      }
    }
    {\fp_to_dim:n {
        \tl_item:nn {#2} {2}
        * \tl_item:nn {#3} {5}
        +
        \tl_item:nn {#2} {4}
        * \tl_item:nn {#3} {6}
        +
        \tl_item:nn {#2} {6}
      }
    }
  }
}
\cs_generate_variant:Nn \compose_transformations:Nnn {cVv,NVv,NVn,NvV,NnV}
\cs_new_nopar:Npn \transform_node:Nn #1#2
{
  \compose_transformations:cVv {pgf@sh@nt@#2} #1 {pgf@sh@nt@#2}
}
\cs_new_nopar:Npn \set_transform_from_node:n #1
{
  \tl_set_eq:Nc \l__sn_transformation_tl {pgf@sh@nt@#1}
  \tikz_scan_point:NNn \l__sn_x_dim \l__sn_y_dim {(#1.center)}

  \dim_set:Nn \l__sn_x_dim {\l__sn_x_dim - \tl_item:cn {pgf@sh@nt@#1}{5}}
  \dim_set:Nn \l__sn_y_dim {\l__sn_y_dim - \tl_item:cn {pgf@sh@nt@#1}{6}}

  \compose_transformations:NnV  \l__sn_transformation_tl {
    {1}{0}{0}{1}{\dim_use:N \l__sn_x_dim}{\dim_use:N \l__sn_y_dim}
  } \l__sn_transformation_tl
}
\cs_generate_variant:Nn \set_transform_from_node:n {v}
\tikzset{
  set~ saved~ nodes~ file~ name/.code={
    \tl_gset:Nx \g__sn_filename_tl {#1}
  },
  transform~ saved~ nodes/.code={
    \set_transform_from_node:v {tikz@last@fig@name}
  },
  set~ node~ group/.code={
    \tl_set:Nn \l__sn_group_tl {#1}
    \pgfkeysalso{
      execute~ at~ end~ scope={
        \maybe_save_nodes:
      }
    }
  },
  save~ nodes~ to~ file/.code={
    \tl_if_eq:nnTF {#1}{false}
    {
      \bool_set_false:N \l__sn_file_bool
    }
    {
      \bool_set_true:N \l__sn_file_bool
    }
    \pgfkeysalso{
      execute~ at~ end~ scope={
        \maybe_save_nodes:
      }
    }
  },
  save~ node/.code={
    \tikz_fig_must_be_named:
    \pgfkeysalso{append~ after~ command={
        \pgfextra{
          \clist_gput_right:Nv \l__sn_nodes_clist {tikz@last@fig@name}
        }
      }
    }
  },
  restore~ nodes~ from~ file/.code={
    \bool_if:NTF \g__sn_preamble_bool
    {
      \restore_nodes_from_file:n {#1}
    }
    {
      \tikz_fig_must_be_named:
      \pgfkeysalso{append~ after~ command={
          \pgfextra{
            \scope
            \split_argument:NNn \tikzset \restore_nodes_from_file:n {#1}
            \endscope
          }
        }
      }
    }
  },
  restore~ nodes~ from~ file/.default = \g__sn_filename_tl,
  restore~ nodes~ from~ list/.code={
    \tikz_fig_must_be_named:
    \pgfkeysalso{append~ after~ command={
        \pgfextra{
          \scope
          \split_argument:NNn \tikzset \restore_nodes_from_list:n {#1}
          \endscope
        }
      }
    }
  }
}
\cs_generate_variant:Nn \clist_gput_right:Nn {Nv}
\cs_new_nopar:Npn \split_argument:NNn #1#2#3
{
  \tl_set:Nx \l__sn_tmpa_tl {\tl_head:n {#3}}
  \tl_if_eq:NNTF \l__sn_tmpa_tl \l__open_bracket_tl
  {
    \split_argument_aux:NNp #1#2#3
  }
  {
    #2 {#3}
  }
}
\cs_new_nopar:Npn \split_argument_aux:NNp #1#2[#3]#4
{
  #1 {#3}
  #2 {#4}
}
\cs_new_nopar:Npn \maybe_save_nodes:
{
  \clist_if_empty:NF \l__sn_nodes_clist
  {
    \bool_if:NTF \l__sn_file_bool
    {
      \save_nodes_to_file:V \l__sn_nodes_clist
    }
    {
      \tl_if_empty:NF \l__sn_group_tl
      {
        \save_nodes_to_list:VV \l__sn_group_tl \l__sn_nodes_clist
      }
    }
    \clist_gclear:N \l__sn_nodes_clist
  }
}
\ExplSyntaxOff
%% 
%% Copyright (C) 2011-2021 by Andrew Stacey <loopspace@mathforge.org>
%% 
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License (LPPL), either
%% version 1.3c of this license or (at your option) any later
%% version.  The latest version of this license is in the file:
%% 
%% http://www.latex-project.org/lppl.txt
%% 
%% This work is "maintained" (as per LPPL maintenance status) by
%% Andrew Stacey.
%% 
%% This work consists of the file  tikzmark.dtx
%% and the derived files           tikzmark.ins,
%%                                 tikzmark.pdf,
%%                                 tikzlibrarytikzmark.code.tex, and
%%                                 tikzmarklibrarylistings.code.tex
%% 
%%
%% End of file `tikzlibrarytikzmark.code.tex'.


==> tikzmarklibrarylistings.code.tex <==
%%
%% This is file `tikzmarklibrarylistings.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tikzmark.dtx  (with options: `listings')
%% ----------------------------------------------------------------
%% tikzmark --- remembering absolute positioning with TikZ.
%% E-mail: loopspace@mathforge.org
%% Released under the LaTeX Project Public License v1.3c or later
%% See http://www.latex-project.org/lppl.txt
%% ----------------------------------------------------------------
%% 
\@ifpackageloaded{listings}{%
  \newif\iflst@linemark
  \lst@linemarktrue
\lst@AddToHook{EveryLine}{%
  \begingroup
  \advance\c@lstnumber by 1\relax
  \pgfmark{line-\lst@name-\the\c@lstnumber-start}%
  \endgroup
}
\lst@AddToHook{EOL}{\pgfmark{line-\lst@name-\the\c@lstnumber-end}%
\global\lst@linemarktrue
}
\lst@AddToHook{OutputBox}{%
  \iflst@linemark
  \pgfmark{line-\lst@name-\the\c@lstnumber-first}%
  \global\lst@linemarkfalse
  \fi
}
\def\tkzmk@lst@fnum#1\relax#2\@STOP{%
  \def\@test{#2}%
  \ifx\@test\@empty
  \def\tkzmk@lst@start{0}%
  \else
  \@tempcnta=#1\relax
  \advance\@tempcnta by -1\relax
  \def\tkzmk@lst@start{\the\@tempcnta}%
  \fi
}
\lst@AddToHook{Init}{%
  \expandafter\tkzmk@lst@fnum\lst@firstnumber\relax\@STOP
  \pgfmark{line-\lst@name-\tkzmk@lst@start-start}%
}
}{%
    \PackageError{tikzmark listings}{The listings package has not been loaded.}{}
}
%% 
%% Copyright (C) 2011-2021 by Andrew Stacey <loopspace@mathforge.org>
%% 
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License (LPPL), either
%% version 1.3c of this license or (at your option) any later
%% version.  The latest version of this license is in the file:
%% 
%% http://www.latex-project.org/lppl.txt
%% 
%% This work is "maintained" (as per LPPL maintenance status) by
%% Andrew Stacey.
%% 
%% This work consists of the file  tikzmark.dtx
%% and the derived files           tikzmark.ins,
%%                                 tikzmark.pdf,
%%                                 tikzlibrarytikzmark.code.tex, and
%%                                 tikzmarklibrarylistings.code.tex
%% 
%%
%% End of file `tikzmarklibrarylistings.code.tex'.

